Probabilistic Model Checking for Continuous Time Markov Chains via Sequential Bayesian Inference

Probabilistic model checking for systems with large or unbounded state space is a challenging computational problem in formal modelling and its applications. Numerical algorithms require an explicit representation of the state space, while statistical approaches require a large number of samples to estimate the desired properties with high confidence. Here, we show how model checking of time-bounded path properties can be recast exactly as a Bayesian inference problem. In this novel formulation the problem can be efficiently approximated using techniques from machine learning. Our approach is inspired by a recent result in statistical physics which derived closed form differential equations for the first-passage time distribution of stochastic processes. We show on a number of non-trivial case studies that our method achieves both high accuracy and significant computational gains compared to statistical model checking.

==> figs_dia/fix_tex_formulae <==
#! /bin/sh

# Note to self:
# If use DIA to edit '*.dia'
# and export to Latex PGF macros (*.tex)
# then run this script, to fix the generated tikzpicture

dia $1.dia -t pgf-tex



ORIGINAL='\\begin{tikzpicture}'
REPLACEMENT='\\begin{tikzpicture}[scale=0.5]'
sed -i 's/'$ORIGINAL'/'$REPLACEMENT'/g' $1.tex



ORIGINAL='\\ensuremath{\\backslash}'
REPLACEMENT='\\'
sed -i 's/'$ORIGINAL'/'$REPLACEMENT'/g' $1.tex

ORIGINAL='\\\$'
REPLACEMENT='$'
sed -i 's/'$ORIGINAL'/'$REPLACEMENT'/g' $1.tex


ORIGINAL='\\{'
REPLACEMENT='\{'
sed -i 's/'$ORIGINAL'/'$REPLACEMENT'/g' $1.tex

ORIGINAL='\\}'
REPLACEMENT='\}'
sed -i 's/'$ORIGINAL'/'$REPLACEMENT'/g' $1.tex


ORIGINAL='\\_'
REPLACEMENT='\_'
sed -i 's/'$ORIGINAL'/'$REPLACEMENT'/g' $1.tex


